Testing Visual Attention in Dynamic Environments

We investigate attention as the active pursuit of useful information. This contrasts with attention as a mechanism for the attenuation of irrelevant information. We also consider the role of short-term memory, whose use is critical to any model incapable of simultaneously perceiving all information on which its output depends. We present several simple synthetic tasks, which become considerably more interesting when we impose strong constraints on how a model can interact with its input, and on how long it can take to produce its output. We develop a model with a different structure from those seen in previous work, and we train it using stochastic variational inference with a learned proposal distribution.

==> RAM-Discussion.tex <==
%!TEX root = RAM-Root.tex

We presented a set of tasks which provide a test-bed for models combining visual attention and sequential prediction. Though simple in form, our family of object detection and tracking tasks can demand sophisticated behavior for consistent success. E.g., to track multiple objects in the presence of distractors, attention must be divided among the target objects while using short-term memory and an understanding of environmental dynamics to estimate the location of objects not currently attended to. We presented a suitable model and some preliminary empirical results showing that our tasks are within reach of current methods, but leave plenty of room to grow.

